Enhancing Genetic Improvement Mutations Using Large Language Models

Large language models (LLMs) have been successfully applied to software engineering tasks, including program repair. However, their application in search-based techniques such as Genetic Improvement (GI) is still largely unexplored. In this paper, we evaluate the use of LLMs as mutation operators for GI to improve the search process. We expand the Gin Java GI toolkit to call OpenAI's API to generate edits for the JCodec tool. We randomly sample the space of edits using 5 different edit types. We find that the number of patches passing unit tests is up to 75% higher with LLM-based edits than with standard Insert edits. Further, we observe that the patches found with LLMs are generally less diverse compared to standard edits. We ran GI with local search to find runtime improvements. Although many improving patches are found by LLM-enhanced GI, the best improving patch was found by standard GI.

==> tables/resultsLSTable.tex <==
\pgfplotstabletypeset[
    col sep=comma,
    column type=r,
    string type,
    columns={EditCategory, Compiled, Passed, Patches, ImprovFound, BestImprov, Median},
    columns/ImprovFound/.style={column name=ImpFound},
    columns/BestImprov/.style={column name=BestImp(ms)},
    columns/Median/.style={column name=Median(ms)},
    every head row/.style={
    before row=\hline,
    after row={
    \hline
    },
    },	% style the first row
    every last row/.style={after row=\hline},	% style the last row
    every column/.style={column type/.add={}{|}},
    every first column/.style={column type/.add={|}{}},	% style the first column
    ]
{data/processedLS.csv}


==> tables/resultsTable.tex <==
\pgfplotstabletypeset[
    col sep=comma,
    column type=r,
    string type,
    columns={EditCategory, UniqueValid, UniqueCompiled, UniquePassed, UniquePatches, Valid, Compiled, Passed, Patches},
    columns/UniqueValid/.style={column name=Valid},
    columns/UniqueCompiled/.style={column name=Compiled},
    columns/UniquePassed/.style={column name=Passed},
    columns/UniquePatches/.style={column name=Patches},
    every head row/.style={
    before row=\hline,
    after row={
    \hline
    & \multicolumn{4}{c|}{Unique} & \multicolumn{4}{c|}{}\\
    \hline
    },
    },	% style the first row
    every last row/.style={after row=\hline},	% style the last row
    every column/.style={column type/.add={}{|}},
    every first column/.style={column type/.add={|}{}},	% style the first column
    ]
{data/processed.csv}

